Approximation Algorithms for the UAV Path Planning with Object Coverage Constraints

We study the problem of the Unmanned Aerial Vehicle (UAV) such that a specific set of objects needs to be observed while ensuring a quality of observation. Our goal is to determine the shortest path for the UAV. This paper proposes an offline algorithm with an approximation of $(2+2n)(1+\epsilon)$ where $\epsilon >0$ is a small constant, and $n$ is the number of objects. We then propose several online algorithms in which objects are discovered during the process. To evaluate the performance of these algorithms, we conduct experimental comparisons. Our results show that the online algorithms perform similarly to the offline algorithm, but with significantly faster execution times ranging from 0.01 seconds to 200 seconds. We also show that our methods yield solutions with costs comparable to those obtained by the Gurobi optimizer that requires 30000 seconds of runtime.

==> biblio <==
% Generated by IEEEtran.bst, version: 1.14 (2015/08/26)
\begin{thebibliography}{10}
\providecommand{\url}[1]{#1}
\csname url@samestyle\endcsname
\providecommand{\newblock}{\relax}
\providecommand{\bibinfo}[2]{#2}
\providecommand{\BIBentrySTDinterwordspacing}{\spaceskip=0pt\relax}
\providecommand{\BIBentryALTinterwordstretchfactor}{4}
\providecommand{\BIBentryALTinterwordspacing}{\spaceskip=\fontdimen2\font plus
\BIBentryALTinterwordstretchfactor\fontdimen3\font minus \fontdimen4\font\relax}
\providecommand{\BIBforeignlanguage}[2]{{%
\expandafter\ifx\csname l@#1\endcsname\relax
\typeout{** WARNING: IEEEtran.bst: No hyphenation pattern has been}%
\typeout{** loaded for the language `#1'. Using the pattern for}%
\typeout{** the default language instead.}%
\else
\language=\csname l@#1\endcsname
\fi
#2}}
\providecommand{\BIBdecl}{\relax}
\BIBdecl

\bibitem{uav_structureinspection}
W.~Jing, D.~Deng, Y.~Wu, and K.~Shimada, ``Multi-uav coverage path planning for the inspection of large and complex structures,'' in \emph{2020 IEEE/RSJ International Conference on Intelligent Robots and Systems (IROS)}.\hskip 1em plus 0.5em minus 0.4em\relax IEEE, 2020, pp. 1480--1486.

\bibitem{smart_farm}
A.~D. Boursianis, M.~S. Papadopoulou, P.~Diamantoulakis, A.~Liopa-Tsakalidi, P.~Barouchas, G.~Salahas, G.~Karagiannidis, S.~Wan, and S.~K. Goudos, ``Internet of things (iot) and agricultural unmanned aerial vehicles (uavs) in smart farming: A comprehensive review,'' \emph{Internet of Things}, vol.~18, p. 100187, 2022.

\bibitem{fire_detect}
C.~Yuan, Z.~Liu, and Y.~Zhang, ``Learning-based smoke detection for unmanned aerial vehicles applied to forest fire surveillance,'' \emph{Journal of Intelligent \& Robotic Systems}, vol.~93, no.~1, pp. 337--349, 2019.

\bibitem{uav_cinema}
I.~Mademlis, V.~Mygdalis, N.~Nikolaidis, and I.~Pitas, ``Challenges in autonomous uav cinematography: An overview,'' in \emph{2018 IEEE international conference on multimedia and expo (ICME)}.\hskip 1em plus 0.5em minus 0.4em\relax IEEE, 2018, pp. 1--6.

\bibitem{civil_security}
H.~Hildmann and E.~Kovacs, ``Using unmanned aerial vehicles (uavs) as mobile sensing platforms (msps) for disaster response, civil security and public safety,'' \emph{Drones}, vol.~3, no.~3, p.~59, 2019.

\bibitem{multi_polygon}
J.~Xie, L.~R.~G. Carrillo, and L.~Jin, ``Path planning for uav to cover multiple separated convex polygonal regions,'' \emph{IEEE Access}, vol.~8, pp. 51\,770--51\,785, 2020.

\bibitem{RRT}
S.~M. LaValle \emph{et~al.}, ``Rapidly-exploring random trees: A new tool for path planning,'' 1998.

\bibitem{math-planning}
J.~De~Waen, H.~T. Dinh, M.~H.~C. Torres, and T.~Holvoet, ``Scalable multirotor uav trajectory planning using mixed integer linear programming,'' in \emph{2017 European conference on mobile robots (ECMR)}.\hskip 1em plus 0.5em minus 0.4em\relax IEEE, 2017, pp. 1--6.

\bibitem{Lyapunov}
J.~Zhang, J.~Yan, P.~Zhang, and X.~Kong, ``Design and information architectures for an unmanned aerial vehicle cooperative formation tracking controller,'' \emph{IEEE Access}, vol.~6, pp. 45\,821--45\,833, 2018.

\bibitem{bio-planning}
Z.~Sun, J.~Wu, J.~Yang, Y.~Huang, C.~Li, and D.~Li, ``Path planning for geo-uav bistatic sar using constrained adaptive multiobjective differential evolution,'' \emph{IEEE Transactions on Geoscience and Remote Sensing}, vol.~54, no.~11, pp. 6444--6457, 2016.

\bibitem{NN-planning1}
M.~M. Kurdi, A.~K. Dadykin, I.~Elzein, and I.~S. Ahmad, ``Proposed system of artificial neural network for positioning and navigation of uav-ugv,'' in \emph{2018 Electric Electronics, Computer Science, Biomedical Engineerings' Meeting (EBBT)}.\hskip 1em plus 0.5em minus 0.4em\relax IEEE, 2018, pp. 1--6.

\bibitem{NN-planning2}
Y.~Zhang, Y.~Zhang, Z.~Liu, Z.~Yu, and Y.~Qu, ``Line-of-sight path following control on uav with sideslip estimation and compensation,'' in \emph{2018 37th Chinese Control Conference (CCC)}.\hskip 1em plus 0.5em minus 0.4em\relax IEEE, 2018, pp. 4711--4716.

\bibitem{q-learning-planning}
T.~Zhang, X.~Huo, S.~Chen, B.~Yang, and G.~Zhang, ``Hybrid path planning of a quadrotor uav based on q-learning algorithm,'' in \emph{2018 37th Chinese control conference (CCC)}.\hskip 1em plus 0.5em minus 0.4em\relax IEEE, 2018, pp. 5415--5419.

\bibitem{g-learning-planning}
S.~Luan, Y.~Yang, H.~Wang, B.~Zhang, B.~Yu, and C.~He, ``3d g-learning in uavs,'' in \emph{2017 12th IEEE Conference on Industrial Electronics and Applications (ICIEA)}.\hskip 1em plus 0.5em minus 0.4em\relax IEEE, 2017, pp. 953--957.

\bibitem{DRL}
L.~He, N.~Aouf, and B.~Song, ``Explainable deep reinforcement learning for uav autonomous path planning,'' \emph{Aerospace science and technology}, vol. 118, p. 107052, 2021.

\bibitem{DRL2}
R.~Xie, Z.~Meng, L.~Wang, H.~Li, K.~Wang, and Z.~Wu, ``Unmanned aerial vehicle path planning algorithm based on deep reinforcement learning in large-scale and dynamic environments,'' \emph{IEEE Access}, vol.~9, pp. 24\,884--24\,900, 2021.

\bibitem{k-means-planning}
X.~Yue and W.~Zhang, ``Uav path planning based on k-means algorithm and simulated annealing algorithm,'' in \emph{2018 37th Chinese Control Conference (CCC)}.\hskip 1em plus 0.5em minus 0.4em\relax IEEE, 2018, pp. 2290--2295.

\bibitem{cellular}
L.~Nam, L.~Huang, X.~J. Li, and J.~Xu, ``An approach for coverage path planning for uavs,'' in \emph{2016 IEEE 14th international workshop on advanced motion control (AMC)}.\hskip 1em plus 0.5em minus 0.4em\relax IEEE, 2016, pp. 411--416.

\bibitem{river_rescue}
P.~Yao, Z.~Xie, and P.~Ren, ``Optimal uav route planning for coverage search of stationary target in river,'' \emph{IEEE Transactions on Control Systems Technology}, vol.~27, no.~2, pp. 822--829, 2017.

\bibitem{surveillance}
M.~Petrl{\'\i}k, V.~Von{\'a}sek, and M.~Saska, ``Coverage optimization in the cooperative surveillance task using multiple micro aerial vehicles,'' in \emph{2019 IEEE International Conference on Systems, Man and Cybernetics (SMC)}.\hskip 1em plus 0.5em minus 0.4em\relax IEEE, 2019, pp. 4373--4380.

\bibitem{hetero-cover}
J.~Chen, F.~Ling, Y.~Zhang, T.~You, Y.~Liu, and X.~Du, ``Coverage path planning of heterogeneous unmanned aerial vehicles based on ant colony system,'' \emph{Swarm and Evolutionary Computation}, vol.~69, p. 101005, 2022.

\bibitem{wsn}
D.~Alejo, J.~A. Cobano, G.~Heredia, J.~R. Mart{\'\i}nez-de Dios, and A.~Ollero, ``Efficient trajectory planning for wsn data collection with multiple uavs,'' in \emph{Cooperative Robots and Sensor Networks 2015}.\hskip 1em plus 0.5em minus 0.4em\relax Springer, 2015, pp. 53--75.

\bibitem{seuwsn}
J.~Huang, F.~Shan, R.~Xiong, Y.~Shao, and J.~Luo, ``Energy-efficient uav flight planning for a general poi-visiting problem with a practical energy model,'' in \emph{2021 International Conference on Computer Communications and Networks (ICCCN)}.\hskip 1em plus 0.5em minus 0.4em\relax IEEE, 2021, pp. 1--10.

\bibitem{straightwsn}
J.~Gong, T.-H. Chang, C.~Shen, and X.~Chen, ``Flight time minimization of uav for data collection over wireless sensor networks,'' \emph{IEEE Journal on Selected Areas in Communications}, vol.~36, no.~9, pp. 1942--1954, 2018.

\bibitem{multi-agent-catastrophe}
D.~Vallejo, J.~J. Castro-Schez, C.~Glez-Morcillo, and J.~Albusac, ``Multi-agent architecture for information retrieval and intelligent monitoring by uavs in known environments affected by catastrophes,'' \emph{Engineering Applications of Artificial Intelligence}, vol.~87, p. 103243, 2020.

\bibitem{bio-inspired}
Q.~Yang and S.-J. Yoo, ``Optimal uav path planning: Sensing data acquisition over iot sensor networks using multi-objective bio-inspired algorithms,'' \emph{IEEE access}, vol.~6, pp. 13\,671--13\,684, 2018.

\bibitem{robotcover}
V.~An, Z.~Qu, and R.~Roberts, ``A rainbow coverage path planning for a patrolling mobile robot with circular sensing range,'' \emph{IEEE Transactions on Systems, Man, and Cybernetics: Systems}, vol.~48, no.~8, pp. 1238--1254, 2017.

\bibitem{DFJ-tsp}
G.~Dantzig, R.~Fulkerson, and S.~Johnson, ``Solution of a large-scale traveling-salesman problem,'' \emph{Journal of the operations research society of America}, vol.~2, no.~4, pp. 393--410, 1954.

\bibitem{MTZ-tsp}
C.~E. Miller, A.~W. Tucker, and R.~A. Zemlin, ``Integer programming formulation of traveling salesman problems,'' \emph{Journal of the ACM (JACM)}, vol.~7, no.~4, pp. 326--329, 1960.

\bibitem{GB-tsp}
B.~Gavish and S.~C. Graves, ``The travelling salesman problem and related problems,'' 1978.

\bibitem{GP-tsp}
L.~Gouveia and J.~M. Pires, ``The asymmetric travelling salesman problem and a reformulation of the miller--tucker--zemlin constraints,'' \emph{European Journal of Operational Research}, vol. 112, no.~1, pp. 134--146, 1999.

\bibitem{nearest-tsp}
M.~Bellmore and G.~L. Nemhauser, ``The traveling salesman problem: a survey,'' \emph{Operations Research}, vol.~16, no.~3, pp. 538--558, 1968.

\bibitem{cheapest-insertion}
T.~Nicholson, ``A sequential method for discrete optimization problems and its application to the assignment, travelling salesman, and three machine scheduling problems,'' \emph{IMA Journal of Applied Mathematics}, vol.~3, no.~4, pp. 362--375, 1967.

\bibitem{genetic-tsp}
J.~H. Holland, \emph{Adaptation in natural and artificial systems: an introductory analysis with applications to biology, control, and artificial intelligence}.\hskip 1em plus 0.5em minus 0.4em\relax MIT press, 1992.

\bibitem{deploy}
W.~Wang, H.~Dai, C.~Dong, F.~Xiao, J.~Zheng, X.~Cheng, G.~Chen, and X.~Fu, ``Deployment of unmanned aerial vehicles for anisotropic monitoring tasks,'' \emph{IEEE Transactions on Mobile Computing}, 2020.

\bibitem{appro-alg}
V.~V. Vazirani, \emph{Approximation algorithms}.\hskip 1em plus 0.5em minus 0.4em\relax Springer, 2001, vol.~1.

\bibitem{Steiner-tree-np-hard}
R.~M. Karp, ``Reducibility among combinatorial problems,'' in \emph{Complexity of computer computations}.\hskip 1em plus 0.5em minus 0.4em\relax Springer, 1972, pp. 85--103.

\bibitem{1.5TSP}
N.~Christofides, ``Worst-case analysis of a new heuristic for the travelling salesman problem,'' Carnegie-Mellon Univ Pittsburgh Pa Management Sciences Research Group, Tech. Rep., 1976.

\bibitem{Dijkstra}
E.~W. Dijkstra \emph{et~al.}, ``A note on two problems in connexion with graphs,'' \emph{Numerische mathematik}, vol.~1, no.~1, pp. 269--271, 1959.

\bibitem{Steiner-tree}
L.~Kou, G.~Markowsky, and L.~Berman, ``A fast algorithm for steiner trees,'' \emph{Acta informatica}, vol.~15, no.~2, pp. 141--145, 1981.

\bibitem{approximation_algorithm}
D.~P. Williamson and D.~B. Shmoys, \emph{The design of approximation algorithms}.\hskip 1em plus 0.5em minus 0.4em\relax Cambridge university press, 2011.

\bibitem{Gurobi}
\BIBentryALTinterwordspacing
{Gurobi Optimization, LLC}, ``{Gurobi Optimizer Reference Manual},'' 2022. [Online]. Available: \url{https://www.gurobi.com}
\BIBentrySTDinterwordspacing

\end{thebibliography}

